An output scaling layer boosts deep neural networks for multiscale ODE systems

Simulating complex diffusion-reaction systems is often prohibitively expensive due to the high dimensionality and stiffness of the underlying ODEs, where state variables may span tens of orders of magnitude. Deep learning has recently emerged as a powerful tool in scientific computing, achieving remarkable progress in modeling and sampling stiff systems. However, data scaling techniques remain largely underexplored, despite their crucial role in addressing the frequency bias of deep neural networks when handling multi-magnitude or high-frequency data. In this work, we propose the Generalized Box-Cox Transformation (GBCT), a novel nonlinear scaling method designed to mitigate multiscale challenges by rescaling inherent multi-magnitude components toward a more consistent order of magnitude. We integrate GBCT into our previous data-driven framework and evaluate its performance against the original baseline surrogate model across six representative scenarios: a 21-species chemical reaction kinetics, a 13-isotope nuclear reaction model, the well-known Robertson problem coupled with diffusion, and practically relevant simulations of two-dimensional turbulent reaction-diffusion systems as well as one- and two-dimensional nuclear reactive flows. Numerical experiments demonstrate that GBCT reduces prediction errors by up to two orders of magnitude compared with the baseline model - particularly in the long-term evolution of dynamical systems - and achieves comparable performance with only about one-sixth of the training epochs. Frequency analysis further reveals that GBCT rescales high-frequency components of the objective function toward lower frequencies to align with the neural network's natural low frequency bias, thereby boosting training and generalization. The source code to reproduce the results in this paper is available at https://github.com/Seauagain/GBCT.

==> text/0_abstract.tex <==

\begin{abstract}

Simulating complex diffusion-reaction systems is computationally intensive due to the high dimensionality and stiffness of ordinary differential equations (ODEs) driven by reaction source terms. While deep learning has been employed to accelerate reaction kinetics computations, challenges such as data scaling and cross-scenario generalization persist, stemming from the multi-scale nature of these dynamical systems. We propose a Generalized Box-Cox Transformation (GBCT) integrated into a deep neural network framework to mitigate multi-scale effects via a data preprocessing approach. GBCT maps physical quantities spanning multiple orders of magnitude onto a unified scale and transforms the strongly nonlinear Arrhenius equation into a near-linear form, enhancing neural network training stability and enabling robust long-term predictions of reaction dynamics. Additionally, we introduce a data generation strategy using Monte Carlo sampling and ODE trajectory augmentation, which ensures flow-condition independence and broad phase-space coverage. Numerical experiments of both chemical and nuclear reacting flows, including pure kinetic predictions and one- and two-dimensional reaction-diffusion scenarios, demonstrate the method’s robustness under highly stiff conditions.



\end{abstract}
%%%%% end %%%%%%%%%%%



%%%%% AMS/PACs/Keywords %%%%%%%%%%%
%\pac{}
% \ams{52B10, 65D18, 68U05, 68U07} 
% \keywords{reaction dynamics, surrogate model, deep learning, data processing, physics}       
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% for the CiCP[J] 


%% Keywords
%% keywords here, in the form: keyword \sep keyword
%% PACS codes here, in the form: \PACS code \sep code
%% MSC codes here, in the form: \MSC code \sep code
%% or \MSC[2008] code \sep code (2000 is the default)

\begin{keword}
deep learning \sep ordinary differential equations \sep multiscale sampling \sep high dimension
\end{keyword}


